Faster Approximate All Pairs Shortest Paths

The all pairs shortest path problem (APSP) is one of the foundational problems in computer science. For weighted dense graphs on $n$ vertices, no truly sub-cubic algorithms exist to compute APSP exactly even for undirected graphs. This is popularly known as the APSP conjecture and has played a prominent role in developing the field of fine-grained complexity. The seminal result of Seidel uses fast matrix multiplication (FMM) to compute APSP on unweighted undirected graphs exactly in $\tilde{O}(n^{\omega})$ time, where $\omega=2.372$. Even for unweighted undirected graphs, it is not possible to obtain a $(2-\epsilon)$-approximation of APSP in $o(n^\omega)$ time. In this paper, we provide a multitude of new results for multiplicative and additive approximations of APSP in undirected graphs for both unweighted and weighted cases. We provide new algorithms for multiplicative 2-approximation of unweighted graphs: a deterministic one that runs in $\tilde{O}(n^{2.072})$ time and a randomized one that runs in $\tilde{O}(n^{2.032})$ on expectation improving upon the best known bound of $\tilde{O}(n^{2.25})$ by Roditty (STOC, 2023). For $2$-approximating paths of length $\geq k$, $k \geq 4$, we provide the first improvement after Dor, Halperin, Zwick (2000) for dense graphs even just using combinatorial methods, and then improve it further using FMM. We next consider additive approximations, and provide improved bounds for all additive $\beta$-approximations, $\beta \geq 4$. For weighted graphs, we show that by allowing small additive errors along with an $(1+\epsilon)$-multiplicative approximation, it is possible to improve upon Zwick's $\tilde{O}(n^\omega)$ algorithm. Our results point out the crucial role that FMM can play even on approximating APSP on unweighted undirected graphs, and reveal new bottlenecks towards achieving a quadratic running time to approximate APSP.

==> abstract_arxiv_1920.tex <==
The all pairs shortest path problem (APSP) is one of the foundational problems in computer science. For weighted dense graphs on $n$ vertices, no truly sub-cubic algorithms exist to compute APSP exactly even for undirected graphs. This is popularly known as the APSP conjecture and has played a prominent role in developing the field of fine-grained complexity. The seminal result of Seidel uses fast matrix multiplication (FMM) to compute APSP on unweighted undirected graphs exactly in $\tilde{O}(n^{\omega})$ time, where $\omega=2.372$. Even for unweighted undirected graphs, it is not possible to obtain a $(2-\epsilon)$-approximation of APSP in $o(n^\omega)$ time. 

In this paper, we provide a multitude of new results for multiplicative and additive approximations of APSP in undirected graphs for both unweighted and weighted cases. We provide new algorithms for multiplicative 2-approximation of unweighted graphs: a deterministic one that runs in $\tilde{O}(n^{2.072})$ time and a randomized one that runs in $\tilde{O}(n^{2.032})$ on expectation improving upon the best known bound of $\tilde{O}(n^{2.25})$ by Roditty (STOC, 2023). For $2$-approximating paths of length $\geq k$, $k \geq 4$, we provide the first improvement after Dor, Halperin, Zwick (2000) for dense graphs even just using combinatorial methods, and then improve it further using FMM. We next consider additive approximations, and provide improved bounds for all additive $\beta$-approximations, $\beta \geq 4$. For weighted graphs, we show that by allowing small additive errors along with an $(1+\epsilon)$-multiplicative approximation, it is possible to improve upon Zwick's $\tilde{O}(n^\omega)$ algorithm. Our results point out the crucial role that FMM can play even on approximating APSP on unweighted undirected graphs, and reveal new bottlenecks towards achieving a quadratic running time to approximate APSP.


==> hardness.tex <==
\section{Subcubic Equivalences of Exact and Approximate Problems}
\label{sec:subcubic-equivalences}

In this section, we give several simple reductions showing that for several important graph and matrix problems, a strong additive approximation is fine-grained equivalent to solving the problem exactly.

\subsection{Subcubic Equivalence of Exact and Approximate \texorpdfstring{\minplus}{(min, +)} Product}

We begin with the \minplus product, sometimes also called the distance product.
Here, we are able to essentially give a full characterization of what additive approximations are possible.

\begin{definition}
    \label{def:min-plus-product}
    Let $A \in \Z^{n \times m}$ and $B \in \Z^{m \times p}$ be integer matrices.
    The {\bf \minplus-product} denoted $A * B$ is an $n \times p$ integer matrix with the following entries,
    \begin{equation*}
        (A * B)_{i, j} = \min_{k \in [m]} a_{i, k} + b_{k, j}
    \end{equation*}
\end{definition}

The \minplus product can be computed in $O(nmp)$ time for arbitrary rectangular matrices.
If $A, B$ are both square matrices of size $n \times n$, this implies a $O(n^3)$ algorithm.
Vassilevska-Williams and Williams \cite{williams2010subcubic} showed that any truly subcubic algorithm would imply a truly subcubic APSP algorithm.
We will show a simple reduction that to some extent additive approximations are equivalent to computing an exact solution, and should therefore also have no truly subcubic algorithm.

\begin{definition}
    \label{def:approx-min-plus-product}
    Let $A \in \Z^{n \times m}$ and $B \in \Z^{m \times p}$ be integer matrices.
    $\hat{C}$ is an {\bf $(\alpha, \beta)$-approximate \minplus product} of $A, B$ if,
    \begin{equation*}
        (A*B)_{i, j} \leq \hat{C}_{i, j} \leq \alpha (A*B)_{i, j} + \beta
    \end{equation*}
    for all $(i, j) \in [n] \times [p]$.
\end{definition}

\begin{proposition}
    Let $\varepsilon > 0$.
    Let $A, B \in \Z^{n \times n}$ be integer matrices with entries bounded by $M = \max(\norm{A}{\infty}, \norm{B}{\infty})$.
    Suppose $M \leq 2 n^l$ is polynomial in $n$.
    If there is algorithm $\innerAlg$ computing a $(1, \beta)$-approximate \minplus product of integer matrices $A, B$ in time $T(n)$ for $\beta \leq n^{l - \varepsilon}$, 
    then there is an algorithm computing the \minplus product for all integer matrices satisfying $\norm{A}{\infty} \leq n^{\varepsilon}$ in time $O(T(n) + n^2 \log n)$.
\end{proposition}

\begin{figure}[H]
\begin{algorithm}[H]
\caption{$\alg{SmallMinPlus}(A, B)$ 
\\ Input: Integer matrices $A, B \in \Z^{n \times n}$ such that $\norm{A}{\infty}, \norm{B}{\infty} \leq n^{\varepsilon}$
\\ Parameters: Maximum entry bound $\varepsilon > 0$ 
\\ Output: \minplus product $A * B$
} 
\label{alg:small-min-plus}
\begin{algorithmic}
\State Define $s$ the smallest integer larger than $\beta$
\State Define $A'$ such that $A'_{i, j} \gets s A_{i, j}$
\State Define $B'$ such that $B'_{i, j} \gets s B_{i, j}$
\State $\hat{C} \gets \innerAlg(A', B', \varepsilon)$
\State construct $C$ such that $C_{i, j} \gets \floor{\frac{\hat{C}_{i, j}}{s}}$
\State \Return $C$
\end{algorithmic}
\end{algorithm}
\end{figure}

\begin{proof}
    First we verify correctness.
    Note $A', B'$ have bounded norm $\norm{A'}{\infty}, \norm{B'}{\infty} \leq s n^{\varepsilon} \leq (\beta + 1) \varepsilon \leq n^{l} + n^{\varepsilon} \leq 2 n^l$.
    By the correctness of the additive approximation sub-routine,
    \begin{equation*}
        (A' * B')_{i, j} \leq \hat{C}_{i, j} \leq (A' * B')_{i, j} + \beta
    \end{equation*}

    Observe that $A' * B'$ is simply $A * B$ scaled up,
    \begin{equation*}
        (A' * B')_{i, j} = \min_{k} A'_{i, k} + B'_{k, j} = s \min_{k} A_{i, k} + B_{k, j} = s(A * B)_{i, j}
    \end{equation*}

    Then,
    \begin{equation*}
        s (A*B)_{i, j} = (A' * B')_{i, j} \leq \hat{C}_{i. j} \leq (A' * B')_{i, j} + \beta = s (A*B)_{i, j} + \beta
    \end{equation*}

    Dividing through by $s$,
    \begin{equation*}
        (A * B)_{i, j} \leq \frac{\hat{C}_{i, j}}{s} \leq (A * B)_{i, j} + \frac{\beta}{s} < (A * B)_{i, j} + 1
    \end{equation*}

    Since $A * B$ is integer valued, $\floor{\frac{\hat{C_{i, j}}}{s}} = (A * B)_{i, j}$.

    It is clear that every step other than the call to $\innerAlg$ requires $n^2 \log n$ time, where we assume the entries are polynomial in $n$ so that $l$ is a constant.
    In particular, operations on numbers of size at most $n^l$ require $O(l \log n) = O(\log n)$ time.
\end{proof}

In particular, achieving any additive approximation better than $n^{l - \varepsilon}$ in subcubic time implies a subcubic algorithm for computing the exact min plus product for matrices with entries bounded by $n^{\varepsilon}$.
This immediately implies that computing a $M^{1 - \varepsilon}$ additive approximation for arbitrary matrices with $\norm{A}{\infty} \leq M$ is subcubically equivalent to an exact computation of the \minplus product, as $M^{\varepsilon} \rightarrow \infty$ for arbitrary $M$.

\begin{corollary}
Let $\varepsilon > 0$.
Suppose there is an algorithm computing a $(1, M^{1 - \varepsilon})$-approximate \minplus product in $T(n, M)$ time given $\norm{A}{\infty}, \norm{B}{\infty} = O(M)$.
Then, the \minplus product of arbitrary matrices with maximum entry $\norm{A}{\infty}, \norm{B}{\infty} \leq M'$ can be computed in $O\left(T\left(n, M'^{\frac{1}{\varepsilon}}\right) + \frac{\log M'}{\varepsilon} n^2 \right)$ time.

In particular, a subcubic $(1, M^{1 - \varepsilon})$-approximation algorithm implies a subcubic algorithm for the \minplus product of arbitrary matrices.
\end{corollary}

\begin{proof}
    It suffices to show that the size of the entries do not increase too much in the scaling step.
    In particular, given matrices with maximum entry at most $M'$, we scale them up to matrices of weight at most $M$ such that $M^{\varepsilon} > M'$.
    In particular, the maximum bit length of any entry is,
    \begin{equation*}
        \log M \leq O\left( \frac{1}{\varepsilon} \log M' \right)
    \end{equation*}

    and we can multiply $\log M$ bit numbers in $O(\log M)$ time.
\end{proof}

Note that Alon, Galil, Margalit showed that sub-cubic \minplus product can be computed for matrices with values at most $n^{3 - \omega}$ \cite{alon1997exponent}.
Then, any additive approximation beating $n^{l - (3 - \omega)}$ for some $l$ implies sub-cubic algorithms for a larger range of matrix values.

Furthermore, there is a simple argument showing that any arbitrary finite approximation of the \minplus product is at least as hard as the boolean matrix multiplication problem, and thus requires $O(n^{\omega})$-time.

\begin{proposition}
    (Folklore) Let $A, B \in \Z^{n \times n}$ be integer matrices with bounded norm, $\norm{A}{\infty}, \norm{B}{\infty} \leq M$. 
    Suppose an algorithm $\innerAlg$ outputs an $(\alpha, \beta)$-approximate \minplus product of $A, B$ in time $T(n)$.
    Then, there is an algorithm $\outerAlg$ computing the matrix product of boolean matrices in $O(T(n) + n^2)$ time.
\end{proposition}

\begin{proof}
    Let $X, Y \in \set{0, 1}^{n \times n}$ be arbitrary boolean matrices.
    Consider the matrices following matrices $A, B$,
    \begin{align*}
        A_{i, j} &= \begin{cases}
        M & X_{i, j} = 1 \\
        \infty & X_{i, j} + 0
        \end{cases} \\
        B_{i, j} &= \begin{cases}
        M & Y_{i, j} = 1 \\
        \infty & Y_{i, j} + 0
        \end{cases}
    \end{align*}
    
    so that,
    \begin{align*}
        (A * B)_{i, j} = \begin{cases}
            2M & (XY)_{i, j} = 1 \\
            \infty & (XY)_{i, j} = 0
        \end{cases}
    \end{align*}

    In particular, given $A, B$, algorithm $\innerAlg$ outputs $\hat{C}$ such that
    \begin{equation*}
        (A * B)_{i, j} \leq \hat{C}_{i, j} \leq \alpha (A * B)_{i, j} + \beta
    \end{equation*}

    Thus, $\outerAlg$ outputs $(XY)_{i, j} = 1$ where $\hat{C}_{i, j}$ finite and $(XY)_{i, j} = 0$ otherwise.
    Note that constructing $A, B$ and reading $\hat{C}$ require $O(n^2)$ time.
\end{proof}

Finally, we show that it is indeed possible to achieve an $o(M)$ additive approximation of the \minplus product in $O(n^{\omega + \varepsilon})$ time for arbitarily small $\varepsilon > 0$. 
In particular, we can achieve sub-linear additive approximation in sub-cubic time.
The approach closely follows that of Zwick \cite{zwick2002bridgingsets}.
We provide the algorithm and analysis for completeness.

\begin{theorem}
\label{thm:min-plus-additive}
Let $\varepsilon \geq 0$ denote the desired approximation parameter. Let $l \in \Z_{+}$.
Given two integer matrices $A, B$ such that $\norm{A}{\infty}, \norm{B}{\infty} \leq n^l$, Algorithm \ref{alg:min-plus-additive} computes a $(1, n^{l - \varepsilon})$-approximate \minplus product in time $O\left( n^{\omega + \varepsilon} \right)$.
\end{theorem}

\begin{figure}[H]
\begin{algorithm}[H]
\caption{$\alg{AdditiveApproxMinPlus}(A, B, \varepsilon)$ 
\\ Input: Integer matrices $A, B \in \Z^{n \times n}$ s uch that $\norm{A}{\infty}, \norm{B}{\infty} < n^l$
\\ Parameters: Approximation parameter $\varepsilon > 0$ 
\\ Output: $(1, \varepsilon)$-approximate \minplus product of $A, B$
} 
\label{alg:min-plus-additive}
\begin{algorithmic}
\State $s \gets \floor{\frac{\varepsilon}{2}}$
\State Define $A', B' \in \Z^{n \times n}$ such that $A'_{i, j} = \ceil{\frac{A_{i, j}}{s}}, B'_{i, j} = \ceil{\frac{B_{i, j}}{s}}$
\State $C' \gets \alg{BoundedMinPlus}(A', B')$ 
\State Define $\hat{C} \in \Z^{n \times n}$ such that $\hat{C}_{i, j} = s \times C'_{i, j}$
\State \Return $\hat{C}$
\end{algorithmic}
\end{algorithm}
\end{figure}

\begin{proof}
    Note that we set $s = \floor{\frac{n^{l - \varepsilon}}{2}}$.
    For any entry of $A', B'$, we have,
    \begin{equation*}
        \frac{A_{i, j}}{s} \leq A'_{i, j} \leq \frac{A_{i, j}}{s} + 1
    \end{equation*}

    Thus, for any $i, k, j$,
    \begin{equation*}
        \frac{A_{i, k} + B_{k, j}}{s} \leq \left( A'_{i, k} + B'_{k, j} \right) \leq \frac{A_{i, k} + B_{k, j}}{s} + 2
    \end{equation*}

    In particular, by the correctness of \alg{BoundedMinPlus},
    \begin{equation*}
        (A*B)_{i, j} \leq s C'_{i, j} \leq (A*B)_{i, j} + 2 s
    \end{equation*}

    We conclude with $s \leq \frac{n^{l - \varepsilon}}{2}$.

    To analyze the running time, note that the entries of $A', B'$ are bounded by $n^{l - s_0}$ so that the time required is $n^{\omega + l - s_0} = n^{\omega + \varepsilon}$.
    The remaining steps are efficient and can be performed in quadratic time.
\end{proof}

The algorithm is very similar to the approximate distance product of \cite{zwick2002bridgingsets}, except that we attempt to bound the additive, rather than multiplicative error.
Zwick shows that given matrices with maximum entry $M$, for some resolution parameter $R$ it is possible to achieve a $1 + \frac{4}{R}$ multiplicative approximation in time $\Tilde{O}(R n^{\omega})$.

To compare, we have $M = n^l$, $\frac{R}{M} = \frac{2}{n^{l - \varepsilon}}$ so that $R = 2 n^{\varepsilon}$, so that in $R n^{\omega}$ time we achieve a $\frac{M}{R}$ additive approximation.
In particular, combining the two, it would be possible to find an approximation $\hat{C}$ such that
\begin{equation*}
    C_{i, j} \leq \hat{C}_{i. j} \leq C_{i, j} + \frac{1}{R} \min \left( M, 4C_{i, j} \right)
\end{equation*}

Note that by choosing the scaling factor $s = \floor{\frac{n^{l - \varepsilon}}{c}}$ for a small constant $c$, we can achieve $\frac{M}{cR}$ approximation in $O(n^{\omega})$ time.

\subsection{Subcubic Equivalence of Exact and Approximate Solutions of Many Graph Problems}

Using techniques from the previous section, we can also show that strong additive approximation algorithms for many famous graph problems, including the All Pairs Shortest Path (APSP) Problem, Graph Diameter and Radius problems.

\subsubsection{All Pairs Shortest Path (APSP)}

We begin with the APSP Problem.
Given a (possibly weighted) graph $G = (V, E)$, an algorithm is asked to the shortest distance and path between all pairs of vertices $u, v \in V$.

\begin{definition}
    \label{def:approx-apsp}
    Let $G = (V, E)$ be a weighted, directed graph with no negative cycles.
    Let $\distT: V \times V \rightarrow \R$ denote the shortest distances between pairs of vertices.
    $\hat{\distT}$ is a {\bf $(\alpha, \beta)$-approximate APSP solution} of $G$ if,
    \begin{equation*}
        \distF{G}{u, v} \leq \hat{\distT}(u, v) \leq \alpha \distF{G}{u, v} + \beta
    \end{equation*}
    for all $u, v \in V$.
\end{definition}

\begin{proposition}
    \label{prop:approx-apsp-exact-equivalence}
    Let $\varepsilon > 0$ and $l \in \Z_+$ a positive integer. 
    Let $G = (V, E)$ be a graph with positive integer weights bounded by $[2 n^l]$. 
    Suppose there is an algorithm $\innerAlg$ computing in $T(n, l)$ time a $(1, \beta)$-approximate APSP solution of $G$ for $\beta \leq n^{l - \varepsilon}$.
    Then, for all integer weighted graphs with weights bounded by $n^{\varepsilon}$, we may compute an exact APSP solution in time $O\left( T(n, l) + l n^2 \right)$
\end{proposition}


\begin{figure}[H]
\begin{algorithm}[H]
\caption{$\alg{ScaleGraphWeights}(G, s)$ 
\\ Input: Weighted graph $G = (V, E)$ and integer scaling factor $s$
\\ Output: Weighted graph $G'$ with weights scaled by $s$
} 
\label{alg:scale-graph-weights}
\begin{algorithmic}
\State Define $G' = (V, E, w')$ with weight function $w'(e) \gets s \times w(e)$
\State \Return $G'$
\end{algorithmic}
\end{algorithm}
\end{figure}

\begin{figure}[H]
\begin{algorithm}[H]
\caption{$\alg{SmallWeightAPSP}(A, B)$ 
\\ Input: Graph $G = (V, E)$ with weights $w: E \rightarrow \set{-n^{\varepsilon}, \dotsc, 0, \dotsc, n^{\varepsilon}}$
\\ Parameters: Approximation parameter $\varepsilon > 0$ 
\\ Output: $(1, n^{l - \varepsilon})$-approximate \minplus product of $A, B$
} 
\label{alg:small-weight-apsp}
\begin{algorithmic}
\State Let $s$ be the smallest integer strictly larger than $\beta$
\State $G' \gets \alg{ScaleGraphWeights}(G, s)$
\State $\hat{D} \gets \innerAlg(G)$
\State Define $D$ such that $D(u, v) \gets \floor{\frac{\hat{D}(u, v)}{s}}$
\State \Return D
\end{algorithmic}
\end{algorithm}
\end{figure}

\begin{proof}
First, I claim $\beta \geq 1$. 
Otherwise, since $G$ is integer weighted, an additive $\beta$-approximation implies an exact solution by ignoring the non-integer part.
In particular, we can assume $\beta \in \Z$ is integral, since by keeping only the integer part, the additive error can only decrease and the estimated value cannot be smaller than the true value which is integral.
Thus, we can assume $s \leq 2 \beta$.

Therefore, the weights in $G'$ are integral and bounded by $2 \beta n^{\varepsilon} \leq 2 n^l$.
By the correctness of $\innerAlg$,
\begin{equation*}
    \distF{G'}{u, v} \leq \hat{D}(u, v) \leq \distF{G'}{u, v} + \beta
\end{equation*}

Since $\distF{G'}{u, v} = s \times \distF{G}{u, v}$,
\begin{equation*}
    \distF{G}{u, v} \leq \frac{\hat{D}(u, v)}{s} \leq \distF{G}{u, v} + \frac{\beta}{s} < \distF{G}{u, v} + 1
\end{equation*}

In particular, since $\distF{G}{u, v}$ is integral, $D(u, v) = \distF{G}{u, v}$.

We invoke $\innerAlg$ on an $n$-vertex graph with weights bounded by $n^l$. 
Constructing $G'$ and $D$ require $O(n^2)$ operations on at most $l$-bit numbers.
The overall time required is $O\left( T(n, l) + l n^2 \right)$
\end{proof}

As we saw with the \minplus product, this implies that a $n^{l - \varepsilon}$ additive approximation implies a sub-cubic algorithm for computing the exact APSP solution for graphs with weights bounded by $n^{\varepsilon}$.
In particular, a truly sub-linear additive approximation for arbitrarily weighted graphs would imply that the APSP can be solved in subcubic time.

\begin{corollary}
    Let $\varepsilon > 0$ be any constant.
    Suppose there is an algorithm computing a $(1, M^{1 - \varepsilon})$-approximate APSP solution on graphs with max weight at most $O(M)$ in time $T(n, M)$.
    Then, the APSP problem can be solved on arbitrary graphs with integer weights bounded by $M'$ in time $O\left( T(n, M'^{1/\varepsilon}) + \frac{n^2}{\varepsilon} \log M' \right)$

    In particular, a truly subcubic $(1, M^{1 - \varepsilon})$-approximation algorithm implies a truly subcubic APSP algorithm on integer weighted graphs.
\end{corollary}

\begin{proof}
    In Proposition \ref{prop:approx-apsp-exact-equivalence}, we saw that $M^{1 - \varepsilon}$ approximation in $O(M)$-bounded weight graphs imply exact APSP algorithms for graphs with weight at most $M^{\varepsilon}$.
    In particular, we must find $M$ such that $M^{\varepsilon} \geq M'$.
    Thus, we it suffices to choose $M = O \left( M'^{1/\varepsilon} \right)$.
    To construct the new graph with weights bounded by $M$ and scale back the original answers, we require time $O(n^2 \log M) = O\left(\frac{n^2}{\varepsilon} \log M'\right)$.
    Invoking the approximation algorithm requires $T(n, M'^{1/\varepsilon})$ time, proving the time bound.
\end{proof}

Indeed, we see that a stronger approximation algorithm implies both a faster exact APSP algorithm as well as a wider range of weights under which the APSP problem can be solved in truly subcubic time.

\subsubsection{Generalization to Many Graph Problems}

We will now generalize the above approach to show that sub-linear additive approximations are equivalent to finding an exact solution for a large class of graph problems.
In the following assume that all graphs have integer weights and therefore that the additive approximation error $\beta$ is an integer larger than 1 by the same discussion as in the proof of Proposition \ref{prop:approx-apsp-exact-equivalence}.
A key property used in many of these proofs is that the solution to the problem is witnessed by a collection of edges that is invariant to scaling (for example a shortest path or minimum weight cycle).

\subsubsection{Single Source Shortest Path (SSSP)}

The exact same algorithm and analysis of Algorithm \ref{alg:small-weight-apsp} shows that an additive approximation of the SSSP problem is equivalent to solving the SSSP problem exactly.
However, this is not particularly of interest, a breakthroughh result of Bernstein, Nanongkai, and Wulff-Nilsen recently showed that the SSSP problem on an arbitrary weighted graphs can be solved in near linear time \cite{bernstein2022negative}.

\subsubsection{Diameter}

We begin with the definition of diameter.

\begin{definition}
    \label{def:diameter}
    Let $G = (V, E)$ be a weighted, directed graph.
    The {\bf diameter} of $G$ is 
    \begin{equation*}
        \diamF{G} = \max_{u, v} \distF{G}{u, v}
    \end{equation*}

    Note that $G$ is strongly connected if and only if $\diamF{G} < \infty$.

    $D(G)$ is an {\bf $(\alpha, \beta)$-diameter} of $G$ if,
    \begin{equation*}
        \diamF{G} \leq D(G) \leq \alpha \diamF{G} + \beta
    \end{equation*}
\end{definition}

\begin{proposition}
    \label{prop:diameter-approx-exact-equiv}
    Let $G$ be a graph on $n$ vertices and $m$ edges with weights bounded in absolute value by $2 n^l$. 
    Suppose there is an algorithm $\innerAlg$ that computes the $(1, \beta)$-approximate diameter of $G$ in time $T(n, l)$ with $\beta \leq n^{l - \varepsilon}$.

    Then, we can compute $\diamF{H}$ for all graphs $H$ with maximum weight bounded by $n^{\varepsilon}$ in $O\left( T(n, l) + l m \right)$ time.
\end{proposition}

\begin{proof}
    We can follow the same approach as above. 
    Begin by choosing $s = \beta + 1$ (recall $\beta$ integral) and scale the weights up by $s$, thus computing graph integral $G' \gets \alg{ScaleGraphWeights}(G, s)$.
    The maximum weight of $G'$ is at most $2 \beta n^{\varepsilon} \leq 2 n^l$.
    Apply our $(1, \beta)$ diameter approximation algorithm $\innerAlg$ to find an approximate diameter $\hat{D}$ satisfying,
    \begin{equation*}
        \diamF{G'} \leq \hat{D}(G') \leq \diamF{G'} + \beta 
    \end{equation*}

    Since $\diamF{G'} = s \times \diamF{G}$,
    \begin{equation*}
        \diamF{G} \leq \frac{\hat{D}(G')}{s} < \diamF{G} + 1
    \end{equation*}

    In particular, $\floor{\frac{\hat{D}(G')}{s}} = \diamF{G}$.
    Note in the running time scaling the diameter takes constant time, and scaling the weights requires only $O(l m)$ time rather than $O(l n^2)$.
\end{proof}

\chris{Compare this with additive approximation of \cite{chechik2014approxdiam}. Should show some tightness result.}

\subsubsection{Vertex Eccentricity and Radius}

We begin with the definitions of vertex eccentricity and radius.

\begin{definition}
    \label{def:eccentricity-radius}
    Let $G$ be a weighted, directed graph. 
    Let $v$ be a vertex in $G$.
    The {\bf eccentricity} of $v$ in $G$ is,
    \begin{equation*}
        \eccF{G}{v} = \max_{u} \distF{G}{v, u}
    \end{equation*}

    The {\bf radius} of a graph $G$ is,
    \begin{equation*}
        \radF{G} = \max_{v} \eccF{G}{v}
    \end{equation*}

    Note $G$ is strongly connected if and only if the radius and all eccentricities are finite.

    $E_G: V \rightarrow \R$ is an {\bf $(\alpha, \beta)$-approximate eccentricity} of $G$ if for all $v \in V$,
    \begin{equation*}
        \eccF{G}{v} \leq E_G(v) \leq \alpha \eccF{G}{v} + \beta 
    \end{equation*}

    Similarly, $R(G)$ is an {\bf $(\alpha, \beta)$-approximate radius} of $G$ if for all $v \in V$,
    \begin{equation*}
        \radF{G} \leq R(G) \leq \alpha \radF{G} + \beta 
    \end{equation*}
\end{definition}

\begin{proposition}
    \label{prop:ecc-approx-exact-equiv}
    Let $G$ be a graph on $n$ vertices and $m$ edges with weights bounded in absolute value by $2 n^l$. 
    Suppose there is an algorithm $\innerAlg$ that computes the $(1, \beta)$-approximate eccentricies of $G$ in time $T(n, l)$ with $\beta \leq n^{l - \varepsilon}$.

    Then, we can compute $\eccT_H$ for all graphs $H$ with maximum weight bounded by $n^{\varepsilon}$ in $O\left( T(n, l) + l (m + n) \right)$ time.
\end{proposition}

\begin{proof}
    As before, choose $s = \beta + 1$ and construct $G' \gets \alg{ScaleGraphWeights}(G, s)$.
    Note that $G'$ has maximum weight at most $s n^{\varepsilon} \leq 2 \beta n^{\varepsilon} \leq 2 n^l$.
    Let $E'_G \gets \innerAlg(G')$. 
    Then, for all $v \in V$,
    \begin{equation*}
        \eccF{G'}{v} \leq E'_G(v) \leq \eccF{G'}{v} + \beta 
    \end{equation*}

    Then, since $\eccF{G'}{v} = s \times \eccF{G}{v}$, we have,
    \begin{equation*}
        \eccF{G}{v} \leq \frac{E'_G(v)}{s} \leq \eccF{G}{v} + \frac{\beta}{s} < \eccF{G}{v} + 1
    \end{equation*}

    Since the edges have integral weight, $\eccF{G}{v} = \floor{\frac{E'_G(v)}{s}}$.
    Scaling weights requires $O(l m)$ time and scaling down eccentricities requires $O(l n)$ time.
\end{proof}

With an identical argument, we can prove the following result for the graph radius problem.

\begin{proposition}
    \label{prop:rad-approx-exact-equiv}
    Let $G$ be a graph on $n$ vertices and $m$ edges with weights bounded in absolute value by $2 n^l$. 
    Suppose there is an algorithm $\innerAlg$ that computes the $(1, \beta)$-approximate radius of $G$ in time $T(n, l)$ with $\beta \leq n^{l - \varepsilon}$.

    Then, we can compute $\radF{H}$ for all graphs $H$ with maximum weight bounded by $n^{\varepsilon}$ in $O\left( T(n, l) + l m \right)$ time.
\end{proposition}

\subsubsection{Girth}

Next, we extend our results to the closely related problems of minimum weight cycle and girth.

\begin{definition}
    \label{def:girth}
    Let $G$ be a weighted, directed graph with weight function $\wt$.
    A {\bf cycle} C is a sequence of vertices $v_1, v_2, \dotsc, v_k = v_1$ such that $(v_i, v_{i + 1}) \in E$ for all $1 \leq i \leq k - 1$ and every vertex appears in the sequence at most once.
    The {\bf girth} of $G$ is,
    \begin{equation*}
        \girthF{G} = \min_{C} \sum_{e \in C} \wt(e)
    \end{equation*}
    
    $\hat{G}$ is an {\bf $(\alpha, \beta)$-girth} if,
    \begin{equation*}
        \girthF{G} \leq \hat{G} \leq \alpha \girthF{G} + \beta 
    \end{equation*}
\end{definition}

\begin{proposition}
    Let $G$ be a graph on $n$ vertices and $m$ edges with weights bounded in absolute value by $2n^l$.
    Suppose there is an algorithm $\innerAlg$ that computes the $(1, \beta)$-approximate girth of $G$ in time $T(n, l)$ with $\beta \leq n^{l - \varepsilon}$.

    Then, we can compute $\girthF{H}$ for all integer-weighted graphs $H$ with maximum weight bounded by $n^{\varepsilon}$ in $O(T(n, l) + lm)$ time.
\end{proposition}

\begin{proof}
    Choose $s = \beta + 1$ and construct $G' \gets \alg{ScaleGraphWeights}(G, s)$.
    Note that $G'$ has maximum weight at most $sn^{\varepsilon} \leq 2 \beta n^{\varepsilon} \leq 2 n^l$.
    Let $\hat{C} \gets \innerAlg(G')$.
    Thus, by the assumption on $\innerAlg$,
    \begin{equation*}
        \girthF{G'} \leq \hat{C} \leq \girthF{G'} + \beta 
    \end{equation*}

    Furthermore, since scaling preserves the relative weights of cycles, $\girthF{G'} = s \times \girthF{G}$,
    \begin{equation*}
        \girthF(G) \leq \frac{\hat{C}}{s} \leq \girthF{G} + \frac{\beta}{s} < \girthF{G} + 1
    \end{equation*}

    Since $\girthF{G}$ has integral value, $\floor{\frac{\hat{C}}{s}} = \girthF{G}$.

    Note that to construct $G'$ requires $O(l m)$ time and scaling down $\hat{C}$ can be done in $O(l)$ time.
\end{proof}

\subsubsection{Minimum and Maximum Cut}

Next, we extend our techniques beyond shortest path and shortest-path related graph parameters as we saw above.
Specifically, we show that strongly sublinear additive approximations of minimum and maximum cut are equivalent to solving the problem exactly on graphs with small weights.

\begin{definition}
    \label{def:min-max-cut}
    Let $G$ be a weighted, directed graph.
    A cut of $G$ is a partition of the vertices into two sets $(S, T)$.
    The {\bf weight} of a cut $(S, T)$ is,
    \begin{equation*}
        \wt(S, T) = \sum_{(u, v) \in E, u \in S, v \in T} \wt(e)
    \end{equation*}

    The {\bf minimum cut} is a cut $(S_{\min}, T_{\min})$, such that $\wt(S_{\min}, T_{\min}) \leq \wt(S, T)$ for all cuts $(S, T)$.
    Conversly, the {\bf maximum cut} is a cut $(S_{\max}, T_{\max})$ such that $\wt(S_{\max}, T_{\max}) \geq \wt(S, T)$ for all cuts $(S, T)$.

    $\hat{C}_{\min}$ is an {\bf $(\alpha, \beta)$-approximate minimum cut} if,
    \begin{equation*}
        \wt(S_{\min}, T_{\min}) \leq \wt(\hat{C}_{\min}) \leq \alpha \wt(S_{\min}, T_{\min}) + \beta 
    \end{equation*}

    Similarly, $\hat{C}_{\max}$ is an {\bf $(\alpha, \beta)$-approximate maximum cut} if,
    \begin{equation*}
        \alpha \wt(S_{\max}, T_{\max}) - \beta \leq \wt(\hat{C}_{\min}) \leq \wt(S_{\max}, T_{\max})
    \end{equation*}
\end{definition}

\begin{proposition}
    Let $G$ be a graph on $n$ vertices and $m$ edges with weights bounded in absolute value by $2n^l$.
    Suppose there is an algorithm $\innerAlg$ that computes the $(1, \beta)$-approximate minimum cut (resp. maximum cut) of $G$ in time $T(n, l)$ with $\beta \leq n^{l - \varepsilon}$.

    Then, we can compute $(S_{\min}, T_{\min})$ (resp. $(S_{\max}, T_{\max})$) for all integer-weighted graphs $G$ with maximum weight bounded by $n^{\varepsilon})$ in $O(T(n, l) + l(m))$.
\end{proposition}

\begin{proof}
    We will show the proof for the maximum cut.
    Choose $s = \beta + 1$ and construct $G' \gets \alg{ScaleGraphWeights}(G, s)$.
    Note that $G'$ has maximum weight at most $sn^{\varepsilon} \leq 2 \beta n^{\varepsilon} \leq 2 n^l$.
    Let $\hat{C} \gets \innerAlg(G')$.
    Thus, by the assumption on $\innerAlg$,
    \begin{equation*}
        \wt(S'_{\max}, T'_{\max}) - \beta \leq \hat{C} \leq \wt(S'_{\max}, T'_{\max})
    \end{equation*}

    Furthermore, since scaling preserves the relative weights of cuts, $\wt(S'_{\max}, T'_{\max}) = s \times \wt(S_{\max}, T_{\max})$,
    \begin{equation*}
        \wt(S_{\max}, T_{\max}) - 1 < \wt(S_{\max}, T_{\max}) - \frac{\beta}{s} \leq \frac{\hat{C}}{s} \leq \wt(S_{\max}, T_{\max})
    \end{equation*}

    Since $\girthF{G}$ has integral value, $\ceil{\frac{\hat{C}}{s}} = \wt(S_{\max}, T_{\max})$.
    The proof for minimum cut follows similarly, except we take $\floor{\frac{\hat{C}}{s}}$.

    Note that to construct $G'$ requires $O(l m)$ time and scaling down $\hat{C}$ can be done in $O(l)$ time.
\end{proof}

In particular, any $(1, \beta)$ approximation of max-cut with $\beta \leq n^{l - \varepsilon}$ is NP-complete by the NP-completeness of the max-cut problem itself.
Of course, much better (constant) conditional upper bounds are known for the max-cut problem \cite{haastad2001some} \cite{khot2007optimal}.

\subsubsection{Main Equivalence Theorem}

Thus we have arrived at the main statement for this section:
Strongly Sub-linear Additive Approximations are Fine-Grained Equivalent to the Exact Problem.

\begin{theorem}
    \label{thm:main-scaling-thm}
    For the following problems, a strongly sub-linear additive approximation implies an efficient algorithm for graphs with small weights.
    Formally, if an $T(n, l)$-time algorithm exists that finds a $\beta \leq n^{l - \varepsilon}$ additive approximation for graphs with maximum weight $O(n^l)$, then there is an $O(T(n, l) + l n^2)$-time algorithm computing the exact solution on graphs with maximum weight $n^{\varepsilon}$.
    \begin{enumerate}
        \item All Pairs Shortest Path
        \item Single Source Shortest Path
        \item Diameter
        \item Vertex Eccentricity
        \item Radius
        \item Girth
        \item Minimum Cut
        \item Maximum Cut
    \end{enumerate}

    In particular, if there is an $(1, M^{1 - \varepsilon})$-approximation algorithm in time $T(n, \log M)$ for graphs with weight $M$, an exact solution on graphs with weight $M'$ can be computed in time $O\left( T \left( n, \frac{1}{\varepsilon} \log M' \right) + \frac{\log M'}{\varepsilon} n^2 \right)$.
\end{theorem}

==> tech-overview.tex <==
\section{Technical Overview}

In the following section, we provide a high level overview of the techniques used by our algorithms.

\subsubsection{Degree Decomposition and Approximate All Pairs Shortest Paths}

We begin by briefly recapping the powerful idea of degree decomposition in computing APSP approximations.
This was first initiated by the work of Aingworth, Chekuri, Indyk, and Motwani \cite{aingworth1999fast}, who pioneered the application of the high-degree low-degree technique in computing approximate APSP solutions.
The idea is roughly as follows.
If we consider all vertices with degree at least $n^{1/2}$, there will be a small set $D$ of size $n^{1/2}$ such that every vertex of high degree has a neighbor in $D$ or is itself in $D$.
$D$ is known as a dominating set.
We compute exact distances from $D$, and then for each pair of vertices, we can take the minimum length path passing through a vertex in $D$.
On paths with high degree vertices, we obtain a $+2$ approximation as $D$ is adjacent to some vertex in the shortest path $P$.
On the other hand, for each pair of vertices whose shortest path contains no high degree vertices, we can compute APSP in time $O(n^{5/2})$ by computing $\bfs$ from every vertex on the graph $G' \subset G$ containing only edges adjacent to low degree vertices.

Expanding this idea to arbitrary degree thresholds $s_1, s_2, \dotsc, s_{k - 1}$ (above we used only $s_1 = n^{1/2}$), Dor, Halperin, and Zwick \cite{dor2000apasp} obtain a $+2$ approximation in time $O(n^{7/3})$ and more generally obtain a $+k$ approximation in time
\begin{equation*}
    \min \left( n^{2 - \frac{2}{k + 2}} m^{\frac{2}{k + 2}}, n^{2 + \frac{2}{3k - 2}} \right)
\end{equation*}

In the sparse case, the algorithm incurs $+2$ error for every degree threshold.
Roughly speaking, as the sizes of the dominating sets increase, we are more restricted on the size of the graph on which we can execute $\dijkstra$.
At each degree threshold, we need to bypass a {\it blocking vertex} via its dominating vertex, incurring a additive error for the extra edge travelled.

In the dense case we can use upper bounds on the size of the dominating sets to add edges that allow us to blocking vertices at intermediate levels of the degree decomposition.
Since the performance of the algorithm can be roughly bounded by $n^2 s_{k - 1}$, being able to add more degree thresholds implies a more efficient algorithm.
This same observation implies that there are more efficient algorithms if the additive approximation requirements are relaxed.

We give a (worst case) example of executing Dor et al.'s algorithm on length 5 paths in \Cref{fig:dhz-example-intro}.

\begin{figure}[ht]
\centering
\includegraphics[width=0.9\textwidth]{images/intro_diagrams/dhz-intro.pdf}
\caption{Example execution of Dor et al.'s \cite{dor2000apasp} algorithm}
\label{fig:dhz-example-intro}
\end{figure}

\subsubsection{New Applications of Rectangular \texorpdfstring{\minplus}{(min, +)} Product}

Previously, Deng et al. \cite{deng2022apasp} observed that if the vertices in the graph are ordered in an Euler tour, the matrices in the product would in fact be bounded difference matrices, and therefore admit fast matrix multiplication algorithms.
Combining this idea with the $\sparseAPASP$ algorithm of Dor, Halperin, and Zwick \cite{dor2000apasp}, they obtained an improvement on the $\denseAPASP$ algorithm of Dor et al. \cite{dor2000apasp} for computing $+2$ additive approximations.
However, using only rectangular matrix multiplication with the exponent $\omega(1, k, 1)$ and the combinatorial $\sparseAPASP$ algorithm, we cannot in fact obtain improvements for additive approximations beyond $+2$, as the combinatorial algorithm $\denseAPASP$ is able to use significantly more degree thresholds, while the techniques of Deng et al. \cite{deng2022apasp} only allow one additional threshold beyond those allowed by $\sparseAPASP$.

By using fast matrix multiplication of arbitrary dimensions, we develop a more general algorithm for multiplying monotone (a generalization of bounded difference) \minplus matrices by extending the work of \cite{chi2022monotone, durr2023rect_monotone} and apply this to obtain improved algorithms for all additive approximations beyond $+2$.
Whereas in $\denseAPASP$ \cite{dor2000apasp} we would like to add edges between dominating sets in a computation of $\dijkstra$, we can instead first use a \minplus product to find the shortest distance using such edges, and then in the invocation of $\dijkstra$ encode these computed distances into the much smaller edge set $u \times V$.
While the new matrices are no longer bounded difference, we can easily ensure that the input matrices are monotone, and therefore apply fast \minplus matrix multiplication \cite{chi2022monotone, durr2023rect_monotone}.
To optimize the performance of our algorithm, we also note that not all the edge sets used in $\denseAPASP$ are necessary, and we compute only those that are minimally necessary to ensure correctness, thus reducing the overall computation time of the \minplus products.

To obtain additive approximations on general graphs, we can use the $\monotoneMinPlus$ algorithm of Chi, Duan, Xie, Zhang \cite{chi2022monotone}.
In some cases, if we only want to compute estimate for short paths (say of some constant length) we can in fact use the more efficient $\boundedMinPlus$ algorithm of Alon, Galil, and Margalit \cite{alon1997exponent}.
This technique is also useful for reducing the maximum degree of the input graph in our multiplicative approximation algorithms.

We give an example of applying rectangular \minplus product to obtain a $+4$ approximation in \Cref{fig:min-plus-intro}.

\begin{figure}[ht]
\centering
\includegraphics[width=0.9\textwidth]{images/intro_diagrams/min-plus-intro.pdf}
\caption{Using \minplus product to replace edge set $D_2 \times D_4$}
\label{fig:min-plus-intro}
\end{figure}

\subsubsection{Low-Depth \texorpdfstring{$\bfs$}{BFS}}

Using the simple yet key observation that small additive errors are only required for short paths to obtain a good multiplicative approximation, Roditty \cite{roditty2023newapasp} obtained a combinatorial algorithm for $(2, 0)$-approximation improving upon Dor et al.'s \cite{dor2000apasp} $+2$ algorithm, which had previously also been the best known multiplicative algorithm.
In particular, observing that length 3 paths are the key computational bottleneck, Roditty used a depth 2 $\bfs$ to efficiently obtain a $+2$ approximation on such paths.

The use of fast matrix multiplication allows us to obtain much stronger bounds on the maximum degree of our input graph such that we can freely compute depth 2 $\bfs$ and in some cases even a depth 3 $\bfs$.
With depth 3 $\bfs$, we also observe that the correctness of our algorithm for paths of 5 edges or less no longer hinges on the number of degree thresholds used, thus allowing us to freely increase the number of degree thresholds and arbitrarily improve the performance of our algorithm.
Indeed, for short paths (length 5 or less) the number of degree thresholds is instead limited by the computation of depth 2 and depth 3 $\bfs$, as these computations become increasingly more expensive with more thresholds.
Nevertheless, using these techniques we are able to obtain a significant improvement in the running time for computing $(2, 0)$-multiplicative approximation for paths of length at most 5.

We give an example when depth 3 $\bfs$ reduces the approximation error in \Cref{fig:bfs-3-intro}.
Compare the following $+4$ approximation to the $+8$ approximation attained by Dor et al.'s algorithm above.

\begin{figure}[ht]
\centering
\includegraphics[width=0.9\textwidth]{images/intro_diagrams/bfs-3-intro.pdf}
\caption{Using depth 3 $\bfs$ to reduce approximation error.}
\label{fig:bfs-3-intro}
\end{figure}

For paths of length more than 6, we can use the techniques mentioned above to compute a $+6$ approximation for paths of any constant length by applying the $\boundedMinPlus$ algorithm of Alon et al. \cite{alon1997exponent}.

\subsubsection{Low-Depth Neighborhoods and Degree Restrictions}

In general, the bottleneck for computing a $(2, 0)$-approximation is accurately estimating the distance of odd length paths.
In particular, we want to obtain $+ \beta$ approximations for paths of length $\beta + 1$.
Indeed, Roditty \cite{roditty2023newapasp} observed that with these techniques, we can then obtain $(2, 0)$-approximations for all paths of length at least $\beta$.

Roditty \cite{roditty2023newapasp} gave a randomized algorithm for computing $+\beta$ approximations on sparse graphs for distances at most $\beta + 2$.
This algorithm mainly uses two ideas.

First, Dor et al.'s algorithm accumulates a $+2$ error for every dominating vertex used in computing the additive approximation.
Since dominating vertices are only used when a blocking edge (roughly speaking, an edge not visible from the current degree threshold) is encountered, short paths are somewhat restricted in how they can accumulate large additive errors.

Second, Roditty extends the hitting set argument to not only consider high degree vertices, but vertices that have large 2-neighborhoods (vertices within distance 2).
Suppose some vertex $u$ has a large 2-neighborhood, so that we can construct a small dominating set $D_1$ of these vertices and compute exact distances from this hitting set.
Then, we have obtained a $+4$ approximation of the shortest path by using the nearest vertex in the dominating set.
On the other hand, if the 2-neighborhood is small, Roditty \cite{roditty2023newapasp} proves that this neighborhood must have a small intersection with dominating set $D_2$ of the next degree threshold.
If the second vertex on the path $u_2$ has degree at least $s_2$, then it has a neighbor in $D_2$, from which we can obtain an accurate additive approximation.
Since the 2-neighborhood has a small intersection with $D_2$, we can efficiently enumerate over all such vertices and take a minimum.
Therefore, we can assume that $u_2$ has degree less than $s_2$.

Using these two ideas Roditty \cite{roditty2023newapasp} obtains a more efficient algorithm for computing $(2, 0)$-approximations for paths of length at least $\beta$.
We extend these techniques to obtain improved combinatorial algorithms on dense graphs for computing $(2, 0)$-approximations on paths of length at least $\beta$.
Combining this with our new applications of fast \minplus matrix multiplication, we obtain further improvements in the performance of the algorithm.

Our combinatorial algorithm uses the following ideas.
First, for shortest paths containing high degree vertices, we use edges between dominating sets to avoid intermediate degree thresholds as inspired by Dor et al.'s $\denseAPASP$ \cite{dor2000apasp}.

Let us then focus on paths containing only low-degree vertices.
Extending the work of Roditty \cite{roditty2023newapasp}, we consider not only 2-neighborhoods, but also 3-neighborhoods, 4-neighborhoods, and indeed neighborhoods up to arbitrary constant depth.
While executing a full $\bfs$ can be expensive, we are only interested in verifying the size of these neighborhoods, so that we can terminate after visiting enough distinct vertices, which is more efficient than a full search of the graph.
Using this technique, we can restrict the degree of almost all vertices on the shortest path.
In fact, the only unconstrained vertices will be the endpoints of the central edge in the path.

In \Cref{fig:degree-restriction-intro}, we give an example of the degree restrictions we can impose when computing $+6$ approximations on length 7 paths.

\begin{figure}[ht]
\centering
\includegraphics[width=0.9\textwidth]{images/intro_diagrams/degree-restrict-intro.pdf}
\caption{Imposing the degree restriction $\level(v_3) \geq 7$}
\label{fig:degree-restriction-intro}
\end{figure}

With the imposed degree restrictions, the central edge can of course still be a blocking edge.
In this case, we employ a depth 2 $\bfs$ to bypass the central edge, and therefore reduce the additive error by avoiding the use of one blocking vertex, as illustrated in \Cref{fig:bfs-2-intro}.

\begin{figure}[ht]
\centering
\includegraphics[width=0.9\textwidth]{images/intro_diagrams/bfs-2-intro.pdf}
\caption{Using depth 2 $\bfs$ to bypass the central edge.}
\label{fig:bfs-2-intro}
\end{figure}

\subsection{Open Questions}

\chris{todo: not sure what to put here?}

\begin{enumerate}
    \item $(2, 0)$-approximation in $\tO{n^2}$ time, combinatorial or using FMM?
    \item Improved combinatorial additive approximation algorithms without path length assumption
    \item Lower Bounds for Approximation and Performance trade-off. Would have to be conditional on $\omega > 2$.
\end{enumerate}

